That Flick is Sick: Gyroscope Integration in Xbox Controllers

Gyroscope integration in Xbox controllers offers new possibilities for enhancing gaming experiences, particularly in first-person shooter (FPS) games. To investigate its potential, we conducted an empirical study with 11 participants, comparing aim precision and reaction times across three input methods: a computer mouse, a standard Xbox controller, and a gyroscope-enabled controller. Participants completed an aim training task, revealing the mouse as the most accurate device, followed by the standard controller. Interestingly, the gyroscope-enabled controller showed reduced accuracy and slower reaction times, attributed to challenges in sensitivity and control. Participant feedback highlighted areas for improvement, including refined sensitivity settings, control stability, and software design. These findings underscore the need for design innovations, such as camera rotation limits and optimized sensitivity thresholds, to make gyroscope-enabled controllers more competitive. Future work should consider diverse gamer profiles and extended evaluation contexts to better understand the role of gyroscopes in gaming interfaces.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
